Higgs Searches in ATLAS

This talk covers the results of a search for the Standard Model Higgs boson in proton-proton collisions with the ATLAS detector at the LHC. The datasets used correspond to integrated luminosities of approximately 4.8 fb-1 collected at sqrt(s) = 7 TeV in 2011 and 5.8 fb-1 at sqrt(s) = 8 TeV in 2012. Individual searches in the channels H->ZZ(*)->4l, H->\gamma\gamma\ and H->WW(*)->e\nu\mu\nu\ in the 8 TeV data are combined with previously published results of searches for H->ZZ(*), WW(*), bb and \tau+\tau- in the 7 TeV data and results from improved analyses of the H->ZZ(*)->4l and H->\gamma\gamma\ channels in the 7 TeV data. Clear evidence for the production of a neutral boson with a measured mass of 126.0 +/- 0.4 (stat) +/- 0.4 (sys) GeV is presented. This observation, which has a significance of 5.9 standard deviations, corresponding to a background fluctuation probability of 1.7 x 10-9, is compatible with the production and decay of the Standard Model Higgs boson. First measurements of the couplings of this particle are presented and are compatible with a SM Higgs boson hypothesis.

==> Makefile <==
LATEX    = latex
# BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = pic2012_A_Schaffer
BASENAMEDISPLAY = pic2012_A_Schaffer

default: full
all : full  display

full:
	latex  ${BASENAME}
	latex  ${BASENAME}
# 	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdfm -p a4  ${BASENAME}

display:
	latex  ${BASENAMEDISPLAY}
	latex  ${BASENAMEDISPLAY}
	latex  ${BASENAMEDISPLAY}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAMEDISPLAY} ${BASENAMEDISPLAY}.pdf

quick:
	latex  ${BASENAME}
	latex  ${BASENAME}
# 	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
        dvipdf -sPAPERSIZE=a4   -dPDFSETTINGS=/prepress ${BASENAME}	
#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

# %.bbl:	%.tex *.bib
# 	$(LATEX) $*
# 	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


